From Persona to Personalization: A Survey on Role-Playing Language Agents

Recent advancements in large language models (LLMs) have significantly boosted the rise of Role-Playing Language Agents (RPLAs), i.e., specialized AI systems designed to simulate assigned personas. By harnessing multiple advanced abilities of LLMs, including in-context learning, instruction following, and social intelligence, RPLAs achieve a remarkable sense of human likeness and vivid role-playing performance. RPLAs can mimic a wide range of personas, ranging from historical figures and fictional characters to real-life individuals. Consequently, they have catalyzed numerous AI applications, such as emotional companions, interactive video games, personalized assistants and copilots, and digital clones. In this paper, we conduct a comprehensive survey of this field, illustrating the evolution and recent progress in RPLAs integrating with cutting-edge LLM technologies. We categorize personas into three types: 1) Demographic Persona, which leverages statistical stereotypes; 2) Character Persona, focused on well-established figures; and 3) Individualized Persona, customized through ongoing user interactions for personalized services. We begin by presenting a comprehensive overview of current methodologies for RPLAs, followed by the details for each persona type, covering corresponding data sourcing, agent construction, and evaluation. Afterward, we discuss the fundamental risks, existing limitations, and future prospects of RPLAs. Additionally, we provide a brief review of RPLAs in AI applications, which reflects practical user demands that shape and drive RPLA research. Through this work, we aim to establish a clear taxonomy of RPLA research and applications, and facilitate future research in this critical and ever-evolving field, and pave the way for a future where humans and RPLAs coexist in harmony.

==> 010acknowledge.tex <==
\section*{Author Contributions}



==> tables/character2.tex <==
\begin{table*}[t]
    \centering
    \small
    \caption{The ways to construct a role-playing agent. \cjj{polish this table. no need to show titles of papers. besides, is this table really necessary? at least, is "models" here really necessary?}} 
    \begin{tabular}{lcc} 
        \toprule 
        Papers & Methods & Models \\ 
        \midrule 
        ChatHaruhi~\cite{li2023chatharuhi} & Prompting \& Fine-tuning & GPT3.5 \& ChatGLM2 \\ 
        \hline
        \makecell[l]{Few-Shot Character Understanding in \\ Movies as an Assessment to Meta-Learning \\ of Theory-of-Mind~\cite{yu2022few}} & Fine-tuning & Longformer-based models \\ 
        \hline
        Generative Agents~\cite{Park2023GenerativeAgents} & Prompting & GPT3.5 \\ 
        \hline
        \makecell[l]{Large Language Models Meet Harry Potter:\\ A Bilingual Dataset for Aligning Dialogue\\ Agents with Characters~\cite{chen2023large}} & Prompting \& Fine-tuning & \makecell{Alpaca \& ChatGLM-6B \\ GPT3 \& GPT3.5 \& ChatGLM} \\ 
        \hline
        \makecell[l]{MBTI Personality Prediction for Fictional \\Characters Using Movie Scripts~\cite{sang2022mbti}} & Fine-tuning & Bert \\ 
        \hline
        \makecell[l]{``Let Your Characters Tell Their Story'':\\ A Dataset for Character-Centric \\Narrative Understanding~\cite{brahman2021let}} & Fine-tuning & \makecell[l]{RoBERTa \& ALBERT \& T5 \\ \& BART \& Longformer} \\
        \hline
        \makecell[l]{Meet Your Favorite Character: Open-domain\\ Chatbot Mimicking Fictional Characters with \\ only a Few Utterances~\cite{han-etal-2022-meet}} & Prompting & Decoder-only transformer \\ 
        \hline
        Character-LLM~\cite{shao2023character} & Fine-tuning & LLaMA-7B \\ 
        \hline
        CharacterGLM~\cite{zhou2023characterglm} & Fine-tuning & ChatGLM \\ 
        \hline
        Thespian~\cite{cui2023thespian} & Fine-tuning & KG-A2C \\ 
        \hline
        RoleLLM~\cite{wang2023rolellm} & Prompting \& Fine-tuning & LLaMA-7B \& GPT3.5 \\
        \hline
        NarrativePlay~\cite{zhao2023narrativeplay} & Prompting  & GPT3.5 \\
        \hline
        CharacterEval~\cite{tu2024charactereval} & Prompting  & \makecell{ChatGLM3-6B \& XVERSE-13B \\ Baichuan2-13B \& Qwen-14B \\ InternLM-20B \& CharacterGLM\\ Xingchen \& Minimax \& BC-NPC-Turbo} \\
        \bottomrule
    \end{tabular}
    \label{tab:character2}
\end{table*}


==> tables/character3.tex <==
\begin{table*}[t]
    \centering
    \small
    \caption{Evaluation of role-playing agents} 
    \begin{tabular}{lccc} 
        \toprule 
        Papers & Methods & Models \\ 
        \midrule 
        ChatHaruhi~\cite{li2023chatharuhi} & Prompting \& Fine-tuning & GPT3.5 \& ChatGLM2 \\ 
        \hline
        \makecell[l]{Few-Shot Character Understanding in \\ Movies as an Assessment to Meta-Learning \\ of Theory-of-Mind~\cite{yu2022few}} & Fine-tuning & Longformer-based models \\ 
        \hline
        Generative Agents~\cite{Park2023GenerativeAgents} & Prompting & GPT3.5 \\ 
        \hline
        \makecell[l]{Large Language Models Meet Harry Potter:\\ A Bilingual Dataset for Aligning Dialogue\\ Agents with Characters~\cite{chen2023large}} & Prompting \& Fine-tuning & \makecell{Alpaca \& ChatGLM-6B \\ GPT3 \& GPT3.5 \& ChatGLM} \\ 
        \hline
        \makecell[l]{MBTI Personality Prediction for Fictional \\Characters Using Movie Scripts~\cite{sang2022mbti}} & Fine-tuning & Bert \\ 
        \hline
        \makecell[l]{``Let Your Characters Tell Their Story'':\\ A Dataset for Character-Centric \\Narrative Understanding~\cite{brahman2021let}} & Fine-tuning & \makecell[l]{RoBERTa \& ALBERT \& T5 \\ \& BART \& Longformer} \\
        \hline
        \makecell[l]{Meet Your Favorite Character: Open-domain\\ Chatbot Mimicking Fictional Characters with \\ only a Few Utterances~\cite{han-etal-2022-meet}} & Prompting & Decoder-only transformer \\ 
        \hline
        Character-LLM~\cite{shao2023character} & Fine-tuning & LLaMA-7B \\ 
        \hline
        CharacterGLM~\cite{zhou2023characterglm} & Fine-tuning & ChatGLM \\ 
        \hline
        Thespian~\cite{cui2023thespian} & Fine-tuning & KG-A2C \\ 
        \hline
        RoleLLM~\cite{wang2023rolellm} & Prompting \& Fine-tuning & LLaMA-7B \& GPT3.5 \\
        \hline
        NarrativePlay~\cite{zhao2023narrativeplay} & Prompting  & GPT3.5 \\
        \hline
        CharacterEval~\cite{tu2024charactereval} & Prompting  & \makecell{ChatGLM3-6B \& XVERSE-13B \\ Baichuan2-13B \& Qwen-14B \\ InternLM-20B \& CharacterGLM\\ Xingchen \& Minimax \& BC-NPC-Turbo} \\
        \bottomrule
    \end{tabular}
    \label{tab:character3}
\end{table*}


==> tables/character4.tex <==




\begin{table}[t]
\centering  
\caption{An overview of different methods for character RPLA construction.}
\label{tab:training_comparison}

\small
\begin{tabular}{p{3.0cm}p{6cm}p{6cm}}
\toprule
\textbf{Training Type} & \textbf{Advantages} & \textbf{Disadvantages} \\
\midrule
\rowcolor[gray]{0.95} \multicolumn{3}{c}{\textit{Parametric Training}} \\
\textbf{Pre-training} & 
\ Simple execution; No more training.  & 
Pre-training . \\ \midrule

\addlinespace[0.25cm]
\textbf{Supervise \hspace{1cm} Fine-Tuning} & 
\ High effectiveness & 
Resource-intensive; Requires training for each character; Training data must be constructed from raw data. \\

\midrule
\rowcolor[gray]{0.95} \multicolumn{3}{c}{\textit{Nonparametric Training}} \\
\textbf{In-context \hspace{1cm} Learning} & 
Balances efficacy and efficiency; No \phantom{more} more training. & 
Challenges the model’s ability to follow instructions; Relies on external databases. \\
\bottomrule
\end{tabular}


\end{table}



